Rovibrational Internal Energy Transfer and Dissociation of High-Temperature Oxygen Mixture

This work constructs a rovibrational state-to-state model for the $\text{O}_2$+$\text{O}_2$ system leveraging high-fidelity potential energy surfaces and quasi-classical trajectory calculations. The model is used to investigate internal energy transfer and non-equilibrium reactive processes in dissociating environment using a master equation approach, whereby the kinetics of each internal rovibrational state is explicitly computed. To cope with the exponentially large number of elementary processes that characterize reactive bimolecular collisions, the internal states of the collision partner are assumed to follow a Boltzmann distribution at a prescribed internal temperature. This procedure makes the problem tractable, reducing the computational cost to a comparable scale with the $\text{O}_2$+O system. The constructed rovibrational-specific kinetic database covers the temperature range of 7500-20000 K. The analysis of the energy transfer and dissociation process in isochoric and isothermal conditions reveals that significant departures from the equilibrium Boltzmann distribution occur during the energy transfer and dissociation phase. Comparing the population distribution of the $\text{O}_2$ molecules against the $\text{O}_2$+O demonstrates a more significant extent of non-equilibrium characterized by a more diffuse distribution whereby the vibrational strands are more clearly identifiable. This is partly due to a less efficient mixing of the rovibrational states, which results in more diffuse rovibrational distributions in the quasi-steady-state distribution. The master equation analysis for the combined $\text{O}_3$+$\text{O}_4$ system reveals that the $\text{O}_2$+$\text{O}_2$ governs the early stage of energy transfer, while the $\text{O}_2$+O takes control of the dissociation dynamics. The findings will provide strong physical foundations for future development of oxygen chemistry.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
